Detecting coherent explorations in SQL workloads

This paper presents a proposal aiming at better understanding a workload of SQL queries and detecting coherent explorations hidden within the workload. In particular, our work investigates SQLShare [11], a database-as-a-service platform targeting scientists and data scientists with minimal database experience, whose workload was made available to the research community. According to the authors of [11], this workload is the only one containing primarily ad-hoc hand-written queries over user-uploaded datasets. We analyzed this workload by extracting features that characterize SQL queries and we show how to use these features to separate sequences of SQL queries into meaningful explorations. We ran several tests over various query workloads to validate empirically our approach.

==> OLDintroduction.tex <==
\section{Introduction}
\label{sec:introduction}



A data exploration is a succession of queries generated by a user in order to detect patterns within the data and eventually acquire new knowledge.
For instance, consider a user analyzing the the sales of a certain product. She may start by displaying the total sales in France. A second query may add a time attribute,   allowing to note that in 2008 the sales plummet. Then, she decides to exhibit the sales to other countries in the same years, looking for drops in sales in other countries. Next queries may focus on specific countries or including more attributes for explaining the phenomenon. %This example illustrates a succession of 3 queries and the knowledge acquire is that there is a widespread sells decrease in 2008. 


%To be able to help the user getting that kind of insight and ease his/her exploration, an approach consists to assess the exploration's and query's quality. Indeed, by doing so, one can solve many problems at once. For example, let's assume that we have a quality score associated with all the explorations and queries. Then, it would be feasible to recommend relevant queries within a current exploration or even detect expert or novice users.
To be able to help the user getting that kind of insight and ease his/her exploration, a first step consists in assessing the quality of the exploration. 
Indeed, quality scores may be used for detecting some patterns of explorations and providing specific suggestions and help.  
Then, it would be feasible to recommend relevant queries within a current exploration or even detect expert or novice users and suggest adapted visualizations.


Our approach is based on the work of Djedaini et al. \cite{DjedainiDLMPV19} 
%An existing work, that is taken as a basis for our studies, is doing this approach 
in the context of OLAP explorations. 
OLAP paradigm brings nice properties such as it's primitive operations, a fixed multi dimensional schema, a fixed query structure and so forth. 
Basically, the entire exploration space available for the user is known in advance as well as the way she is able to explore it. Indeed the user's scope is limited to the cube, and devising queries consists of choosing subsets of the available dimensions, measures and filters. %and all it's group by set in respect of the filters and the measures.


Whereas in SQL, the boundaries are quite fuzzy because the select statement is very permissive if it's not restricted within a framework like OLAP. For instance one could create an entire column that is not present in the database like a distance calculation or a boolean attribute. 
Then our main challenge will be to adapt this Olap work to the sql context meaning that the queries will be formed differently with a vast variety of shapes. Also the features representing the queries will be different. 


%Our proposal includes a model for representing some relevant parts of SQL queries , in the form of and a set of metrics capturing several perspectives of exploration quality. These metrics will be the input for a clustering algorithm, with the goal of detecting similar explorations. We are currently developing an algorithm for extracting query features and computing metrics. The current version, as a proof of concept, focus in one particular query feature and its associated quality metrics.

Our proposal includes (i) a model for representing the more relevant components of SQL queries, called query parts (ex. projections, selections, aggregations) within several SQL syntaxes, (ii) a set of descriptors capturing several perspectives of exploration quality, and
(iii) an algorithm that parses SQL queries and computes descriptors. The current version of the algorithm, as a proof of concept, focus in one particular query part and its associated quality descriptors.




==> clustering.tex <==
\section{Clustering of explorations}
\label{sec:clustering}

\vero{Si on fait quelque chose du genre.}


==> datasets-bis.tex <==
\vero{In addition to} %We first experiment with 
the SQLShare dataset 
\vero{we use} %. We then experiment with 
other datasets for which a ground truth is available \vero{(presented in Subsection \ref{sec:datasets}). Our goal is} %in order 
to better underline the effectiveness of \vero{each method.} %our approach. 
We expect our approach to  find a segmentation that is close to the ground truth.
As one of the datasets also contains timestamps, we  compare to the heuristic used in the literature, i.e., the  30-minutes cutoff.
\vero{Experiments with these datasets also allow the optimization of our proposal (e.g. feature selection) and the tuning of parameters and hyper-parameters.}

%\vero{Then, we experiment with the SQLShare dataset, and finally, we compare our results with other state of the art findings.}

\patrick{Our approach is written in Python 3 with packages: Scikit-learn, Imbalanced-learn \cite{DBLP:journals/jmlr/LemaitreNA17}, Snorkel \cite{DBLP:journals/pvldb/RatnerBEFWR17} 
and py-kmm\footnote{\url{https://github.com/vodp/py-kmm}}.}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Datasets with ground truth}
\label{sec:datasets}



%\subsubsection{Datasets}

We used \vero{two} %three 
real workloads, \vero{consisting of} 
%Two of them are 
logs of multidimensional queries that we have used in our previous works \cite{DBLP:journals/is/DjedainiDLMPV19}. 
\vero{In a preliminary study \cite{DBLP:conf/dolap/PeraltaVRM19}, we used a third dataset, proposed}
%the third one is a log SQL queries used 
for clustering queries in \cite{DBLP:journals/tkde/KulLXCKU18}.
\vero{However, we discarded this dataset because of its quality. Actually, it does not contain real explorations but sets of queries supposed to be similar, and experiments in \cite{DBLP:conf/dolap/PeraltaVRM19} show that it is not appropriate for testing session segmentation.}

We briefly present the datasets  
and we refer the readers to \cite{DBLP:journals/is/DjedainiDLMPV19} %.corresponding articles 
for \vero{further details.} %more precisions.

\paragraph{Datasets description}
The first dataset, named \textit{Open} in what follows, consists of navigation traces collected %\vero{in September 2016}
in the context of a French project on energy vulnerability. 
These traces were produced by 8 volunteer students 
of a Master's degree in Business Intelligence,  
answering  fuzzy information needs defined by their lecturer,
to develop explorative OLAP navigations using Saiku\footnote{http://meteorite.bi/products/saiku} over 
three cubes instances.
The main cube is organized as a star schema with 19 dimensions, 68 (non-top) levels, 24 measures, and contains 37,149 facts recorded in the fact table.
The other cubes are organized in a similar way.
%From this experiment, we could gather $39$ explorations, representing $1608$ queries. THIS WAS THE WHOLE SET BUT WILLEME NEVER CALCULATED THE FEATURES FOR THE REMAINING SESSIONS.
From this experiment, we reuse $16$ sessions, representing $28$ explorations and $941$ queries.
The ground truth is a manual segmentation
made by the lecturer based on some guessed notion of user goal and supported by timestamps. 
Notably, automatic segmentation was not the purpose of the work at the time 
manual segmentation was done.
%At that moment (in 2016), the segmentation of sessions was not a goal; we were informed of this fact.
%\patrick{we could git this btw}  \vero{???}

The second dataset, named \textit{Enterprise}, consists of navigation traces of 14 volunteers among SAP employees, in the context of a previous study on discovering user intents  \cite{DrushkuLMP19}.
%\cite{DBLP:conf/caise/DrushkuALMPD17}.
We set 10 business needs, and volunteers were asked to analyze some of the 7 available data sources to answer each of the 10 business needs, 
using a SAP prototype that supports keyword-based BI queries\footnote{Patent Reference: 14/856,984 : BI Query and Answering using full text search and keyword semantics}. 
In total, this dataset contains $24$ sessions, corresponding to $104$ user explorations and accounting for $525$ queries.
Volunteers were explicitly requested to express to what information needs they were answering,  which constitutes our ground truth for this dataset.



% The third dataset, named \textit{Exam}, consists 
% of queries gathered over $2$ years from 
% student exams at University of Buffalo. Queries correspond to student's answers to $2$ exam questions (one per year). 
% A parser that allow to extract several query parts (including the ones we need) is also available for download. The parser also filters the queries that obtained low grades, proposing a total of $102$ queries.


Notably, in Open and Enterprise datasets, users did not have to write any SQL code,
contrarily to SQLShare. % or Exam. 
Indeed, Saiku and the SAP prototype generated queries from users high-level operations. However, in both cases, users devised real explorations\vero{, taking the time to analyse results before devising new querys}.
\vero{Users of the Open dataset were Master students learning data analysis skills, users of the Enterprise dataset were developers with varied analysis skills, while SQLShare users are anonymous end-users. }
%In the tests conducted over these workloads, we expect our approach to  find a segmentation that is close to the ground truth.
%
% Conversely, queries in the Exam dataset are hand-written, but each student devised only one query. In order to simulate explorations, we made the hypothesis that the answers to a same exam question should  
% mimic students attempts to find the correct answer. To this end, we arranged together the queries that answer a same exam question, obtaining 2 explorations (the ground truth for this dataset). 
%
%In the tests conducted over this workload, we expect our approach to find the point that separates answers to the 2 questions. 

\paragraph{Dataset analysis and feature extraction}
For these two datasets, 
the feature extraction was made as in \cite{DBLP:journals/is/DjedainiDLMPV19}, enriched with detection of the features pertaining to tables (NoT and NCT) \vero{and attributes (NoAt and NCAt)}.
\vero{A WORD ABOUT RED AND JACCARD WITHOUT NoAt CAR TROP CORRELATED. CORRELATIONS CAN COME HERE.}

Table \ref{table:datasets} compares \vero{both} %the three 
datasets in terms of number of sessions, number of explorations (the ground truth), number of queries and summarizes features extraction. \vero{A last column allows the direct comparison with SQLShare features; of course, without lines concerning a ground truth.}
A first remark concerns the length of sessions. The Open dataset contains long sessions concerning few explorations while the Enterprise dataset contains shorter sessions concerning more explorations. 
Sessions length is actually dependent on GUI; while third party OLAP tools, like Saiku, log a new query for each user action (including intermediate drag-and-drops), the SAP prototype only logs final queries. %In the Exam dataset, sessions and explorations were simulated.
Regarding features, queries in \vero{both} %the three 
datasets concern a quite small number of projections, selections, aggregations, %and 
tables \vero{and attributes}. Relative edit distance (RED) and Jaccard index (JI) illustrate that queries are more similar in the Enterprise dataset.% and highly dissimilar in the Exam dataset. The latter observation actually contradicts our hypothesis on the Exam dataset (stating that students' answers to a same exam question should be similar).

\vero{Finally, note that in terms of queries per session, the SQLShare dataset is similar to the Enterprise one, while in terms of features, it has bigger gaps with the other datasets. Specifically, SQLShare queries, in average, are richer in terms of projections (with high variations among queries), but contains less aggregations and tables, being intermediate in terms of selections and attributes. Regarding relative features, except for the number of common projections, and in a lower degree the number of common attributes, most features show that queries are less similar than in the other datasets. }

\begin{table}[]
%\begin{table}[!ht]
\begin{center}
\begin{tabular}{lcc|c}
%& \multicolumn{3}{c}{\textbf{Datasets}} \\
                                  & \textbf{Open}            & \textbf{Enterprise}     & \textbf{SQLShare}          \\
%\hline
Nb of sessions                    & 16              & 24             & 451              \\
Nb of explorations  & 28              & 104            &               \\
Nb of queries                     & 941             & 525            & 10,668            \\
Avg queries per session               & 58         & 21         & 24            \\
Avg queries per explor.               & 34         & 5         &            \\
Avg explor. per session          & 2     & 4    &              \\
%\hline
Avg and range of NoP              & 3.62 {[}1.70{]}  & 2.18 {[}0.60{]} & 7.98 {[}22.32{]}    \\
Avg and range of NoS              & 1.33 {[}0.21{]}  & 0.76 {[}0.30{]} & 1.19 {[}3.10{]} \\
Avg and range of NoA              & 1.34 {[}1.40{]}  & 1.14 {[}0.50{]} & 0.41 {[}2.02{]} \\
Avg and range of NoT              & 3.28 {[}1.70{]}  & 2.03 {[}1.40{]} & 1.50 {[}3.29{]} \\
Avg and range of NoAt             & 8.18 {[}3.02{]}  & 4.23 {[}2.00{]} & 6.65 {[}11.78{]} \\
Avg and range of NCP              & 3.16 {[}0.70{]}  & 1.34 {[}0.40{]} & 4.36 {[}17.53{]} \\
Avg and range of NCS              & 1.13 {[}0.21{]}  & 0.46 {[}0.30{]} & 0.59 {[}1.96{]} \\
Avg and range of NCA              & 1.17 {[}0.40{]}  & 0.77 {[}0.30{]} & 0.20 {[}1.08{]} \\
Avg and range of NCT              & 2.97 {[}0.70{]}  & 1.46 {[}0.40{]} & 0.85 {[}2.05{]} \\
Avg and range of NCAt             & 7.14 {[}3.51{]}  & 2.49 {[}2.21{]} & 2.98 {[}5.36{]} \\
Avg and range of RED              & 3.85 {[}0.19{]}  & 2.09 {[}0.25{]} & 10.90 {[}26.57{]} \\
Avg and range of JI               & 0.57 {[}0.10{]}  & 0.79 {[}0.10{]} & 0.45 {[}0.39{]} \\
\end{tabular}
\caption{Characteristics of \vero{Open, Enterprise and SQLShare} %the 3
datasets}
\label{table:datasets}
\end{center}
\end{table}



\patrick{comment on differences between datasets, particularly feature correlation, see Figure \ref{fig:correlation-sqlshare}, where dopan and smartbi are concatenated (do we need to separate them?)}
\vero{SI ON LE LAISSE ICI, IL FAUDRAIT SEPARER OPEN ET ENTREPRISE, CAR CONCANATED PAS ENCORE DEFINI.}



\begin{figure}
\begin{center}
\includegraphics[width=6cm]{heatmap_correlation_sqlshare.png}
\includegraphics[width=6cm]{heatmap_correlation_dopan_smartbi.png}
\end{center}
\caption{Intrinsic feature correlation in  datasets SQLShare (left) and Concatenate (right).
}
\label{fig:correlation-sqlshare}
\end{figure}


==> datasets.tex <==
\section{Datasets with ground truth}
\label{sec:datasets}

\vero{In addition to} %We first experiment with 
the SQLShare dataset 
\vero{we use} %. We then experiment with 
other datasets for which a ground truth is available. \vero{Our goal is} %in order 
to better underline the effectiveness of our approach, i.e. we expect to find a segmentation that is close to the ground truth.
As one of the datasets also contains timestamps, we  compare to the heuristic used in the literature, i.e., the  30-minutes cutoff.
%\vero{Experiments with these datasets also allow the optimization of our proposal (e.g. feature selection) and the tuning of parameters and hyper-parameters.}
\vero{In addition, these datasets can be used for learning models and tune parameters, as will be explained in Section \ref{sec:sessions}.}

%\patrick{Our approach is written in Python 3 with packages: Scikit-learn, Imbalanced-learn \cite{DBLP:journals/jmlr/LemaitreNA17}, Snorkel \cite{DBLP:journals/pvldb/RatnerBEFWR17} 
%and py-kmm\footnote{\url{https://github.com/vodp/py-kmm}}.}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




%\subsubsection{Datasets}

We used \vero{two} %three 
real workloads, \vero{consisting of} 
%Two of them are 
logs of multidimensional queries that we have used in our previous works \cite{DBLP:journals/is/DjedainiDLMPV19}. 
\vero{In a preliminary study \cite{DBLP:conf/dolap/PeraltaVRM19}, we used a third dataset, proposed}
%the third one is a log SQL queries used 
for clustering queries in \cite{DBLP:journals/tkde/KulLXCKU18}.
\vero{However, we discarded this dataset because of its quality. Actually, it does not contain real explorations but sets of queries supposed to be similar, and experiments in \cite{DBLP:conf/dolap/PeraltaVRM19} show that it is not appropriate for testing session segmentation.}

We briefly present the datasets  
and we refer the readers to \cite{DBLP:journals/is/DjedainiDLMPV19} %.corresponding articles 
for \vero{further details.} %more precisions.

\paragraph{Datasets description}
The first dataset, named \textit{Open} in what follows, consists of navigation traces collected %\vero{in September 2016}
in the context of a French project on energy vulnerability. 
These traces were produced by 8 volunteer students 
of a Master's degree in Business Intelligence,  
answering  fuzzy information needs defined by their lecturer,
to develop explorative OLAP navigations using Saiku\footnote{http://meteorite.bi/products/saiku} over 
three cubes instances.
The main cube is organized as a star schema with 19 dimensions, 68 (non-top) levels, 24 measures, and contains 37,149 facts recorded in the fact table.
The other cubes are organized in a similar way.
%From this experiment, we could gather $39$ explorations, representing $1608$ queries. THIS WAS THE WHOLE SET BUT WILLEME NEVER CALCULATED THE FEATURES FOR THE REMAINING SESSIONS.
From this experiment, we reuse $16$ sessions, representing $28$ explorations and $941$ queries.
The ground truth is a manual segmentation
made by the lecturer based on some guessed notion of user goal and supported by timestamps. 
Notably, automatic segmentation was not the purpose of the work at the time 
manual segmentation was done.
%At that moment (in 2016), the segmentation of sessions was not a goal; we were informed of this fact.
%\patrick{we could git this btw}  \vero{???}

The second dataset, named \textit{Enterprise}, consists of navigation traces of 14 volunteers among SAP employees, in the context of a previous study on discovering user intents  \cite{DrushkuLMP19}.
%\cite{DBLP:conf/caise/DrushkuALMPD17}.
We set 10 business needs, and volunteers were asked to analyze some of the 7 available data sources to answer each of the 10 business needs, 
using a SAP prototype that supports keyword-based BI queries\footnote{Patent Reference: 14/856,984 : BI Query and Answering using full text search and keyword semantics}. 
In total, this dataset contains $24$ sessions, corresponding to $104$ user explorations and accounting for $525$ queries.
Volunteers were explicitly requested to express to what information needs they were answering,  which constitutes our ground truth for this dataset.



% The third dataset, named \textit{Exam}, consists 
% of queries gathered over $2$ years from 
% student exams at University of Buffalo. Queries correspond to student's answers to $2$ exam questions (one per year). 
% A parser that allow to extract several query parts (including the ones we need) is also available for download. The parser also filters the queries that obtained low grades, proposing a total of $102$ queries.


Notably, in Open and Enterprise datasets, users did not have to write any SQL code,
contrarily to SQLShare. % or Exam. 
Indeed, Saiku and the SAP prototype generated queries from users high-level operations. However, in both cases, users devised real explorations\vero{, taking the time to analyse results before devising new querys}.
\vero{Users of the Open dataset were Master students learning data analysis skills, users of the Enterprise dataset were developers with varied analysis skills, while SQLShare users are anonymous end-users and there is no knowledge about their analysis skills. }
%In the tests conducted over these workloads, we expect our approach to  find a segmentation that is close to the ground truth.
%
% Conversely, queries in the Exam dataset are hand-written, but each student devised only one query. In order to simulate explorations, we made the hypothesis that the answers to a same exam question should  
% mimic students attempts to find the correct answer. To this end, we arranged together the queries that answer a same exam question, obtaining 2 explorations (the ground truth for this dataset). 
%
%In the tests conducted over this workload, we expect our approach to find the point that separates answers to the 2 questions. 

\paragraph{Dataset analysis and feature extraction}
For these two datasets, 
the feature extraction was made as in \cite{DBLP:journals/is/DjedainiDLMPV19}, enriched with detection of the features pertaining to tables (NoT and NCT) \vero{and attributes (NoAt% and NCAt
)}.

Table \ref{table:datasets} compares \vero{both} %the three 
datasets in terms of number of sessions, number of explorations (the ground truth), number of queries and summarizes features extraction. \vero{A last column allows the direct comparison with SQLShare features; of course without lines concerning a ground truth.}

A first remark concerns the length of sessions. The Open dataset contains long sessions concerning few explorations while the Enterprise dataset contains shorter sessions concerning more explorations. 
Sessions length is actually dependent on GUI; while third party OLAP tools, like Saiku, log a new query for each user action (including intermediate drag-and-drops), the SAP prototype only logs final queries. %In the Exam dataset, sessions and explorations were simulated.
Regarding features, queries in \vero{both} %the three 
datasets concern a quite small number of projections, selections, aggregations, %and 
tables \vero{and attributes}. 


\vero{In addition, note that in terms of queries per session, the SQLShare dataset is similar to the Enterprise one, while in terms of features, it has bigger gaps with the other datasets. Specifically, SQLShare queries, in average, are richer in terms of projections (with high variations among queries), but contains less aggregations and tables, being intermediate in terms of selections and attributes. 
Regarding relative features, except for the number of common projections, %and in a lower degree the number of common attributes, 
most features show that queries are less similar than in the other datasets. }

Relative edit distance (RED) and Jaccard index (JI) illustrate that queries are more similar in the Enterprise dataset.% and highly dissimilar in the Exam dataset. The latter observation actually contradicts our hypothesis on the Exam dataset (stating that students' answers to a same exam question should be similar).

%\vero{A WORD ABOUT RED AND JACCARD WITHOUT NoAt CAR TROP CORRELATED. CORRELATIONS CAN COME HERE.}

\begin{table}[]
%\begin{table}[!ht]
\begin{center}
\begin{tabular}{lcc|c}
%& \multicolumn{3}{c}{\textbf{Datasets}} \\
                                  & \textbf{Open}            & \textbf{Enterprise}     & \textbf{SQLShare}          \\
%\hline
Nb of sessions                    & 16              & 24             & 451              \\
Nb of explorations  & 28              & 104            &               \\
Nb of queries                     & 941             & 525            & 10,668            \\
Avg queries per session               & 58         & 21         & 24            \\
Avg queries per explor.               & 34         & 5         &            \\
Avg explor. per session          & 2     & 4    &              \\
%\hline
Avg and range of NoP              & 3.62 {[}1.70{]}  & 2.18 {[}0.60{]} & 7.98 {[}22.32{]}    \\
Avg and range of NoS              & 1.33 {[}0.21{]}  & 0.76 {[}0.30{]} & 1.19 {[}3.10{]} \\
Avg and range of NoA              & 1.34 {[}1.40{]}  & 1.14 {[}0.50{]} & 0.41 {[}2.02{]} \\
Avg and range of NoT              & 3.28 {[}1.70{]}  & 2.03 {[}1.40{]} & 1.50 {[}3.29{]} \\
Avg and range of NoAt             & 8.18 {[}3.02{]}  & 4.23 {[}2.00{]} & 6.65 {[}11.78{]} \\
Avg and range of NCP              & 3.16 {[}0.70{]}  & 1.34 {[}0.40{]} & 4.36 {[}17.53{]} \\
Avg and range of NCS              & 1.13 {[}0.21{]}  & 0.46 {[}0.30{]} & 0.59 {[}1.96{]} \\
Avg and range of NCA              & 1.17 {[}0.40{]}  & 0.77 {[}0.30{]} & 0.20 {[}1.08{]} \\
Avg and range of NCT              & 2.97 {[}0.70{]}  & 1.46 {[}0.40{]} & 0.85 {[}2.05{]} \\
Avg and range of NCAt             & 7.14 {[}3.51{]}  & 2.49 {[}2.21{]} & 2.98 {[}5.36{]} \\
Avg and range of RED              & 3.85 {[}0.19{]}  & 2.09 {[}0.25{]} & 10.90 {[}26.57{]} \\
Avg and range of JI               & 0.57 {[}0.10{]}  & 0.79 {[}0.10{]} & 0.45 {[}0.39{]} \\
\end{tabular}
\caption{Characteristics of \vero{Open, Enterprise and SQLShare} %the 3
datasets}
\label{table:datasets}
\end{center}
\end{table}



%\patrick{comment on differences between datasets, particularly feature correlation, see Figure \ref{fig:correlation-sqlshare}, where dopan and smartbi are concatenated (do we need to separate them?)}
%\vero{SI ON LE LAISSE ICI, IL FAUDRAIT SEPARER OPEN ET ENTREPRISE, CAR CONCANATED PAS ENCORE DEFINI.}

\paragraph{Feature correlation}

\vero{In order to complete the analysis of query features in the three datasets, we study their pairwise correlation. We exclude RED and JI features (which are aggregated from the other query parts) and NoCh (which is merely informative). 
Correlation results are shown in Figure \ref{fig:correlation-sqlshare}.}

\vero{
First of all, note that correlations are stronger in the Open and Enterprise datasets than in the SQLShare dataset. Specifically, the stronger correlations are those of NoAt with NoP and NoT. This is partially explained by the type of queries (OLAP-like queries with few selections) and the underlying star-like database schemes. 
Noticeably, the attributes on the query text are mainly the projected attributes and the ones used for joins (and more joins are necessary when more attributes are projected). 
These attributes are less correlated in the SQLShare dataset, where both database schemes and queries are free-style. }
%
\vero{This strong correlation of NoAt with NoP and NoT, happening in the datasets used for learning (see Section \ref{sec:sessions}), reinforce the decision of not including NoAt as a core feature.}

\vero{As expected, there are other lower correlations among absolute and relative features, for example, between NoP and NCP.
}

\vero{The last dataset in Figure \ref{fig:correlation-sqlshare}, called Concatenate, is the union of Open and Enterprise datasets, which is used as training set in our proposal (see Section \ref{sec:sessions}). The correlation among its attributes is very close to the one among attributes in the Open dataset. }


\begin{figure}
\begin{center}
\includegraphics[width=6cm]{correlation-dopan.png}
\includegraphics[width=6cm]{correlation-smartBI.png}

\includegraphics[width=6cm]{correlation-sqlshare.png}
\includegraphics[width=6cm]{correlation-concat.png}
\end{center}
\caption{Feature correlation in  datasets
Open (up left), Enterprise (up right),
SQLShare (bottom left) and Concatenate (bottom right).}
\label{fig:correlation-sqlshare}
\end{figure}


==> old-stuff.tex <==
\section{OLD STUFF}


\section{Experimentation}





\subsection{Exploration extraction}
The explorations are deduced thanks to an assumption we made : queries in the file respect a chronological order. It is not indubitable but it looks like it. Indeed, we notice that there are successions of queries belonging to the same user in the file. Moreover, in most cases, the succession starts with a simple query. Then, from one to another we remark that the next query is a copy of the previous one but with the addition of new fragment (i.e : an other table in the from clause or an another projected attribute) 
In order to confirm, at least to some extent, this hypothesis we did a small experimentation. It consists to check that there is enough legit exploration created that way. In other words, we test that there is not too much very small or very large explorations.
This method yield 452 explorations. We found that on average a session is composed of 22 queries with a standard deviation of 74.9. The minimum and maximum of queries within an exploration is respectively 1 and  937. 
There is 196 explorations with less than 3 queries. We might remove them because of their lack of relevance. In the other hands there is 13 explorations with more than 120 queries. Those explorations are also questionable. In total we have 243 quite legit explorations. 

\patrick{also cite \cite{DBLP:conf/dawak/RomeroMAPB11}
for the idea of separating sessions}

 
